Reverse Bernstein Inequality on the Circle

The more then hundred years old Bernstein inequality states that the supremum norm of the derivative of a trigonometric polynomial of fixed degree can be bounded from above by supremum norm of the polynomial itself. The reversed Bernstein inequality, that we prove in this note, says that the reverse inequality holds for functions in the orthogonal complement of the space of polynomials of fixed degree. In fact, we derived a more general result for the lower bounds on higher derivatives. These bounds are better then those obtained by applying bound for the first derivative successively several times.

==> defs.tex <==
\makeatletter
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Arrows
\newcommand{\into}[1][]{\stackrel{#1}{\hookrightarrow}}
\renewcommand{\to}[1][]{\stackrel{#1}{\rightarrow}}
\newcommand{\too}[1][]{\stackrel{#1}{\longrightarrow}}
\newcommand{\ot}[1][]{\stackrel{#1}{\leftarrow}}
\newcommand{\oot}[1][]{\stackrel{#1}{\longleftarrow}}
\newcommand{\oto}[1][]{\stackrel{#1}{\leftrightarrow}}
\newcommand{\ootoo}[1][]{\stackrel{#1}{\longleftrightarrow}}

% Binary operators
% Brackets
\def\<{\left\langle}
\def\>{\right\rangle}
\let\doublebar=\|
\def\|#1\|{\left\doublebar#1\right\doublebar}
\def\cl#1{\left\lceil#1\right\rceil}
\def\fl#1{\left\lfloor#1\right\rfloor}
\def\dsb#1{[\mkern-5mu[#1]\mkern-5mu]}
\def\st{\;{\bm :}\;}
\def\set#1{\left\{#1\right\}}

% Math Operators
\let\dmo=\DeclareMathOperator
\dmo\dist{\dbf}
\dmo\gcdtmp{\mathsf{gcd}}\let\gcd=\gcdtmp
\dmo\lcm{\mathsf{lcm}}
\dmo\vr{\mathsf{VR}}
\dmo\bc{\mathsf{bc}}
\dmo\dvol{\drm\mathit{vol}}
\dmo\odd{\mathsf{odd}}
\dmo\even{\mathsf{even}}
\dmo\Katz{\mathrm{Katz}}
\dmo\Lip{\mathrm{Lip}}
\dmo\lin{\Lsf}
\dmo\diam{\mathsf{diam}}
\dmo\radius{\mathsf{radius}}
\dmo\Closure{\mathsf{Closure}}
\dmo*\argmax{\mathrm{arg\,max}}
\dmo*\argmin{\mathrm{arg\,min}}
\dmo\id{\mathrm{Id}}\let\Id=\id
\dmo\convexhull{\mathsf{ConvexHull}}\let\ConvexHull=\convexhull
\dmo\d@tmp{\drm\mkern-3mu}\let\d=\d@tmp
\dmo\nbd{\mathsf{Nbd}}\let\Nbd=\nbd
\dmo\Res{\mathrm{Res}}
\dmo\skel{\mathsf{Skel}}
\dmo\Spec{\mathsf{Spec}}\let\spec=\Spec
\dmo\supp{\mathsf{supp}}
\dmo\var{\mathsf{var}}
\dmo\O@{\Ocal}\let\O=\O@
\dmo\o@{\scalebox{0.65}{\Ocal}}\let\o=\o@

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Letters
\let\tmp=\phi \let\phi=\varphi \let\varphi=\tmp
\let\tmp=\epsilon \let\epsilon=\varepsilon \let\varepsilon=\tmp

%% \let\emptyset=\varnothing
\def\imathbf{{\bm\imath}}
\def\jmathbf{{\bm\jmath}}

%% Math letters
%% Define \<letter><font> 
\newcommand{\bmmax}{2}
\usepackage{bm}

\def\mathun#1{\underline{#1}}
\def\mathov#1{\overline{#1}}
\def\mathbar#1{\bar{#1}}
\def\mathhat#1{\hat{#1}}
\def\mathwh#1{\widehat{#1}}
\def\mathtilde#1{\tilde{#1}}


\def\mkmathletter#1#2{%
    \expandafter\gdef\csname#1#2\endcsname%
           {\ensuremath{\csname math#2\endcsname{#1}}}%
}

\edef\letters{a,b,c,d,e,f,g,h,i,j,k,l,m,n,o,p,q,r,s,t,u,v,w,x,y,z}
\edef\Letters{A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}
\edef\Lletters{\letters,\Letters}

\def\mkmathletters#1#2{%
        \@for\ltr:={#2}\do{\expandafter\mkmathletter\ltr{#1}}%
}

\mkmathletters{frak}{\Lletters} %\Afrak, \bfrak
\mkmathletters{bb}{\Letters}    %\Rbb,\Nbb   blackboard bold
\mkmathletters{cal}{\Lletters}   %\Acal,\bcal caligraphic
\mkmathletters{bf}{\Lletters}   %\Abf,\bbf   bold
\mkmathletters{rm}{\Lletters}   %\Arm, \brm  roman
\mkmathletters{sf}{\Lletters}   %\Asf, \bsf  san serif
\mkmathletters{un}{\Lletters}   % underlined
\mkmathletters{ov}{\Lletters}   % overlined
\mkmathletters{wh}{\Lletters}   % with hat
\mkmathletters{hat}{\Lletters}  %
\mkmathletters{tilde}{\Lletters}% with tilde
\mkmathletters{bar}{\Lletters}  % with bar, smaller then overlined

%double tilde
\usepackage{accents}
\newcommand{\dbltilde}[1]{\accentset{\approx}{#1}}

\edef\greek{alpha,beta,gamma,delta,epsilon,zeta,eta,theta,jota,kappa,lambda,%
  mu,nu,xi,pi,omikron,rho,sigma,tau,upsilon,varphi,phi,chi,psi,omega}
\edef\Greek{Alpha,Beta,Gamma,Delta,Epsilon,Zeta,Eta,Theta,Jota,Kappa,%
  Lambda,Mu,Nu,Xi,Pi,Omikron,Rho,Sigma,Tau,Upsilon,Varphi,Phi,Chi,%
  Psi,Omega}
\edef\Ggreek{\greek,\Greek}

\def\mkboldgreek#1;{\expandafter\def\csname#1bf\endcsname{%
    \expandafter\bm\csname#1\endcsname}}

\def\mkbolds#1{%
  \@for\ltr:={#1}\do{\expandafter\mkboldgreek\ltr;}%
}

\def\mksfgreek#1;{\expandafter\def\csname#1sf\endcsname{%
    \expandafter\mathsf{\csname#1\endcsname}}}

\def\mksf#1{%
  \@for\ltr:={#1}\do{\expandafter\mksfgreek\ltr;}%
}

\mkbolds{\Ggreek}
\mksf{\Ggreek}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Debug
\newcommand{\skipthis}[2][]{\relax}
\let\comment=\skipthis

\long\def\coloredtext#1#2{%
  \begingroup%
    \color{#1}%
    #2%
  \endgroup%
}

\long\def\red#1{\coloredtext{red}{#1}}
\long\def\green#1{\coloredtext{green}{#1}}
\long\def\blue#1{\coloredtext{blue}{#1}}
\long\def\cyan#1{\coloredtext{cyan}{#1}}
\long\def\brown#1{\coloredtext{brown}{#1}}
\long\def\green#1{\coloredtext{green}{#1}}
\long\def\lime#1{\coloredtext{lime}{#1}}
\long\def\magenta#1{\coloredtext{magenta}{#1}}
\long\def\olive#1{\coloredtext{olive}{#1}}
\long\def\pink#1{\coloredtext{pink}{#1}}
\long\def\purple#1{\coloredtext{purple}{#1}}
\long\def\teal#1{\coloredtext{teal}{#1}}
\long\def\violet#1{\coloredtext{violet}{#1}}
\long\def\yellow#1{\coloredtext{yellow}{#1}}
\long\def\grey#1{\coloredtext{gray}{#1}}\let\gray=\grey


\long\def\skippar#1\par{\relax\par}
\long\def\justpar#1\par{#1\par}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Theorems,etc

% \newtheorem{Alphastatements}{XXX}
% \def\theAlphastatements{\Alph{Alphastatements}}
% \newtheorem{independent}{XXX}
% \newtheorem{withinsection}{XXX}[section]
% \newtheorem{withinsection1}{XXX}[section]

% \newtheorem{definition}[withinsection]{Definition}
 % \newtheorem{proposition}[withinsection]{Proposition}
% \newtheorem{theorem}[withinsection]{Theorem}
%% \newtheorem{corollary}[withinsection]{Corollary}
 % \newtheorem{lemma}[withinsection]{Lemma}
% \newtheorem{alphatheorem}[Alphastatements]{Theorem}
% \newtheorem{alphaconjecture}[Alphastatements]{Conjecture}
 
% \newtheorem{conjecture}{Conjecture}
% \newtheorem{question}[conjecture]{Question}
% \renewcommand{\theconjecture}{Q\arabic{conjecture}}

\def\eproofsymbol{$\boxtimes$}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%% COMMUTATIVE DIAGRAMS
\usepackage{tikz-cd}\usetikzlibrary{decorations.pathmorphing}
\usepackage{environ}

\tikzset{
  symbol/.style={
    draw=none,
    every to/.append style={
      edge node={node [sloped, allow upside down, auto=false]{$#1$}}}
  }
}
\NewEnviron{skipenv}{\relax}
\newenvironment{cd}[1][]
               {\begin{tikzcd}[ampersand replacement=\&,#1]}
               {\end{tikzcd}}

\newcommand{\cdon}{%
  \renewenvironment{cd}[1][]
                 {\begin{tikzcd}[ampersand replacement=\&,##1]}
                 {\end{tikzcd}}%
}

\newcommand{\cdoff}{%
  \renewenvironment{cd}[1][]
                 {\textcolor{red}{\text{Commutative diagram}}%
                  \begin{skipenv}%
                 }
                 {\end{skipenv}}%
}

%%% COMMUTATIVE DIAGRAMS
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\makeatother

